Mitigating Disparity while Maximizing Reward: Tight Anytime Guarantee for Improving Bandits

We study the Improving Multi-Armed Bandit (IMAB) problem, where the reward obtained from an arm increases with the number of pulls it receives. This model provides an elegant abstraction for many real-world problems in domains such as education and employment, where decisions about the distribution of opportunities can affect the future capabilities of communities and the disparity between them. A decision-maker in such settings must consider the impact of her decisions on future rewards in addition to the standard objective of maximizing her cumulative reward at any time. In many of these applications, the time horizon is unknown to the decision-maker beforehand, which motivates the study of the IMAB problem in the technically more challenging horizon-unaware setting. We study the tension that arises between two seemingly conflicting objectives in the horizon-unaware setting: a) maximizing the cumulative reward at any time based on current rewards of the arms, and b) ensuring that arms with better long-term rewards get sufficient opportunities even if they initially have low rewards. We show that, surprisingly, the two objectives are aligned with each other in this setting. Our main contribution is an anytime algorithm for the IMAB problem that achieves the best possible cumulative reward while ensuring that the arms reach their true potential given sufficient time. Our algorithm mitigates the initial disparity due to lack of opportunity and continues pulling an arm till it stops improving. We prove the optimality of our algorithm by showing that a) any algorithm for the IMAB problem, no matter how utilitarian, must suffer $\Omega(T)$ policy regret and $\Omega(k)$ competitive ratio with respect to the optimal offline policy, and b) the competitive ratio of our algorithm is $O(k)$.

==> sec_OptimalStrategy.tex <==
\subsection{Offline Optimal Algorithm for \imab}
\label{subse: offline optimal}
%\vine{Combine Sections 2 and 3, and title it Model and Preliminaries. The new section will have two subsections: one titled model and the second titled 'Offline Optimal Algorithm for \IMAB'}
%\label{sec: optimal strategy}
In this section, we define the optimal algorithm with respect to which the regret of our algorithm is computed. 
In particular, given the knowledge of the time horizon $T$ and the reward functions $f_i(\cdot)$ of all the arms, we show that the optimal algorithm, i.e., the algorithm that maximizes the cumulative reward over $T$ time steps, always pulls a single arm at all time steps.
We remark that the external regret and policy regret of an algorithm do not coincide even in this case (see Example 1 in \cite{HEIDARI2016}).

Let $\langle k, (f_i)_{i\in [k]} \rangle$ be an instance of the \IMAB problem, let $T$ be the time horizon, and
let $\mathcal{A}$ denote the set of all algorithms for the above instance.
\begin{proposition}
\label{prop: single arm optimal policy}
Let $\alg^* \in \mathcal{A}$ be a policy such that $$\alg^*_t = \arg\max_{i\in[k]} \sum_{t=1}^T f_i(t)$$ for all $t \in [T]$. Then, $\alg^*(T) \geq \alg(T) ~~\text{for all}~~ \alg \in \mathcal{A}.$
\end{proposition}
\gan{ I think this result is already known (Proposition 1 of Heidari et al.)) for known time horizon and the extension to unknown time horizon is immediate. Should we cite Heidari et al's paper here?  }
Proposition \ref{prop: single arm optimal policy} implies that in the offline setting, where the algorithm knows the reward functions of the arms in
the \IMAB instance and the time horizon $T$ beforehand, the optimal strategy is to pull the same arm (as defined above) at all time steps. 
The proof of this proposition uses an exchange argument along with induction and can be found in Appendix \ref{app: proof of offline optimal strategy}.
Recalling our motivating example, we can infer that the strategy that gives maximum returns to the decision-maker entails allocating the entire budget
$B$ to same neighbourhood every fiscal year. 
However, this is highly unfair to other neighbourhoods and 
may lead to further amplification of the already existing disparity among different communities.
%However, it should be clear to the reader that this is highly unfair to other neighbourhoods and may lead to further amplification of the already existing disparity among different communities.
Further, from a practical perspective, a decision-maker is unlikely to have knowledge of $T$ and much less of $f_i$ beforehand.
This leads us on a quest to design an algorithm with \emph{good} performance guarantees in the absence of such knowledge.


\vish{Say that CR is a well studied objective in online algos etc with citations}

\vish{1. Any algo, no matter how utilitarian, suffers linear regret}
\vish{2. Is it enough to look at something simple like RR? Equitable. And linear regret anyway}
\vish{3. RR is equitable but sub optimal competitive ratio}
\vish{4. Can we do better in terms of both fairness and CR? Yes ... Key technical contribution}
